Better Together: Unified Motion Capture and 3D Avatar Reconstruction

We present Better Together, a method that simultaneously solves the human pose estimation problem while reconstructing a photorealistic 3D human avatar from multi-view videos. While prior art usually solves these problems separately, we argue that joint optimization of skeletal motion with a 3D renderable body model brings synergistic effects, i.e. yields more precise motion capture and improved visual quality of real-time rendering of avatars. To achieve this, we introduce a novel animatable avatar with 3D Gaussians rigged on a personalized mesh and propose to optimize the motion sequence with time-dependent MLPs that provide accurate and temporally consistent pose estimates. We first evaluate our method on highly challenging yoga poses and demonstrate state-of-the-art accuracy on multi-view human pose estimation, reducing error by 35% on body joints and 45% on hand joints compared to keypoint-based methods. At the same time, our method significantly boosts the visual quality of animatable avatars (+2dB PSNR on novel view synthesis) on diverse challenging subjects.

==> tables/hand_pose_estimation.tex <==
\begin{table*}[h]

\caption{Hand Pose Estimation evaluation results on MOYO (millimeters, lower is better).}
\label{tab:hand_pose}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lllllllllllllllll}
\toprule
 & & \multicolumn{3}{c}{\textbf{Boat Pose}} & \multicolumn{3}{c}{\textbf{Camel Pose}} & \multicolumn{3}{c}{\textbf{Cobra Pose}} & \multicolumn{3}{c}{\textbf{Firefly Pose}} & \multicolumn{3}{c}{\textbf{Average}} \\
 \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14} \cmidrule(r){15-17} 
\textbf{Method}& \textbf{Keypoints} & \footnotesize{\textit{W-MPJPE}} & \footnotesize{\textit{MPJPE}} & \footnotesize{\textit{PA-MPJPE}} & \footnotesize{\textit{W-MPJPE}} & \footnotesize{\textit{MPJPE}} & \footnotesize{\textit{PA-MPJPE}} & \footnotesize{\textit{W-MPJPE}} & \footnotesize{\textit{MPJPE}} & \footnotesize{\textit{PA-MPJPE}} & \footnotesize{\textit{W-MPJPE}} & \footnotesize{\textit{MPJPE}} & \footnotesize{\textit{PA-MPJPE}} & \footnotesize{\textit{W-MPJPE}} & \footnotesize{\textit{MPJPE}} & \footnotesize{\textit{PA-MPJPE}} \\
\cmidrule(r){1-2} \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14} \cmidrule(r){15-17} 
Ours & Sapiens & \textbf{12.79} & \textbf{9.19} & \textbf{6.29} & \textbf{36.78} & 28.13 & 10.15 & \textbf{16.87} & \textbf{10.73} & \textbf{5.86} & \textbf{20.77} & \textbf{20.02}& 9.33 & \textbf{21.80} & \textbf{17.02} & \textbf{7.91} \\
Ours (kp only) & Sapiens & 17.39 & 13.28 & 7.20 & 56.95 & 23.94 & \textbf{8.83} & 18.30 & 13.54 & 5.49 & 37.93 & 23.88 & 8.54 & 32.64 & 18.66 & 7.52 \\
EasyMocap & Sapiens & 21.70 & 17.84 & 7.63 & 56.33 & \textbf{21.45} & 9.27 & 23.61 & 17.83 & 5.53 & 26.75 & 22.21 & \textbf{5.84} & 32.10 & 19.87 & 7.07 \\ 
EasyMocap & OpenPose & 24.34 & 17.84 & 7.67 & 75.70 & 29.08 & 9.37 & 25.85 & 20.46 & \textbf{5.30} & 281.25 & 53.98 & 11.15 & 101.79 & 30.34 & 8.37 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
